vSkyConf: Cloud-assisted Multi-party Mobile Video Conferencing

As an important application in the busy world today, mobile video conferencing facilitates virtual face-to-face communication with friends, families and colleagues, via their mobile devices on the move. However, how to provision high-quality, multi-party video conferencing experiences over mobile devices is still an open challenge. The fundamental reason behind is the lack of computation and communication capacities on the mobile devices, to scale to large conferencing sessions. In this paper, we present vSkyConf, a cloud-assisted mobile video conferencing system to fundamentally improve the quality and scale of multi-party mobile video conferencing. By novelly employing a surrogate virtual machine in the cloud for each mobile user, we allow fully scalable communication among the conference participants via their surrogates, rather than directly. The surrogates exchange conferencing streams among each other, transcode the streams to the most appropriate bit rates, and buffer the streams for the most efficient delivery to the mobile recipients. A fully decentralized, optimal algorithm is designed to decide the best paths of streams and the most suitable surrogates for video transcoding along the paths, such that the limited bandwidth is fully utilized to deliver streams of the highest possible quality to the mobile recipients. We also carefully tailor a buffering mechanism on each surrogate to cooperate with optimal stream distribution. We have implemented vSkyConf based on Amazon EC2 and verified the excellent performance of our design, as compared to the widely adopted unicast solutions.

==> implementation.tex <==
\secttion{Implementations}



==> system_models.tex <==
\section{System Model}

All the assigned surrogates are connected in a complete graph, noted as $G=(\mathcal{S}, \mathcal{E})$. $\mathcal{S}$ represents the surrogate set, and the surrogates help transcode and relay the video flows among users in the same video conferencing session. Each user can only disseminate and receive the session flows through his own surrogate. $\mathcal{E}$ is the link set composed of the links between each pair of surrogates, with a bounded bandwidth $C_{i,j}$ on link $(i,j)$.

To sustain stable video sessions between each pair of users, we apply a constant bit rate (CBR) transcoding style, to avoid disrupt quality degradation caused by bit rate surges in the same session. Any video session can be transcoded into different qualities at different bitrates, with the larger bitrates representing the better qualities. Generally, a session stream with a higher bitrate can only be down-sampled at a lower bitrate, but not in reverse, since up-sampling provides no quality improvements but consumes unnecessary precious bandwidths. 
%Transcoding is a complicated work, with various compression algorithms focusing on different aspects. To avoid jerky effects caused by inappropriate frame drops usually applied in temporal compressions, in our paper, we only allow intra-frame spacial compressions to guarantee a smooth user experience by retaining the frame rates, though the session window dimensions and the video fidelities within a frame are likely affected.

Due to the heterogeneities of end devices' capabilities and transient connection conditions, the download capacities of each end user vary over the time. Still, different layouts of the multi-session visual chats lead to customizable realignments and resizings for each single session, and we denote the requested maximal bit rate for the session originating from user $m$ to user $n$ as $R^{m,n}$, which act as an upper bound for the active receive session bit rate of session $m \rightarrow n$, {\em i.e.}, $r^{m,n}$. Let $I^{m,n}_{i,j}$ indicate whether session $m \rightarrow n$ traverses through the link $(i,j)$.

Let $c^m_{ij}$ denotes the actual flow rates on link $(i,j)$ originating from user $m$ and can be transcoded into lower bitrates by any intermediate surrogates. Let $l_{i,j}$ denote the link latency of $(i,j)$. $T_i(r_1, r_2)$ denotes the transcoding latency from source rate $r_1$ to $r_2$ at surrogate $s_i$ , where $r1 > r2$. No transcoding is needed if $r_1 = r_2$, and the latency is $0$.

The quality of experiences for session originating from $m$ perceived by user $n$ are characterized by an increasing function, {\em i.e.}, $U(\frac{r_{m,n}}{R_{m,n}})$. The problem can be formulated into Eqn.~\ref{eqn:optimization}. The objective is to maximize the overall utility in an established video conference. $L^{m,n}$ is the maximal bearable latency for session $m \rightarrow n$.

   \begin{equation}
			\begin{array}{l}
				max \mathop{\sum}\limits_{m, n \in \mathcal{S}, m \neq n} U (\frac{r^{m,n}}{R^{m,n}}) \\
				s.t. \\
						\begin{array}{l}
							\sum_{i:(i,j) \in \mathcal{E}} I^{m,n}_{i,j} - \sum_{k:(j,k) \in \mathcal{E}} I^{m,n}_{j,k} = b^{m,n}_j  \forall j, m,n \in \mathcal{S}, m \neq n\\
							I^{m,n}_{i,j} \times r^{m,n}\leq c^m_{i,j}, \forall (i,j) \in \mathcal{E}, m,n \in \mathcal{S}, m \neq n \\
							\sum_{m \in \mathcal{S}} c^m_{i,j} \leq C_{i,j}, \forall (i,j) \in \mathcal{E} \\
							\sum_{(i,j) \in \mathcal{E}} I^{m,n}_{i,j} \times l_{i,j} = \alpha (m,n,i,j) \\
							\sum_{i,k:(i,j), (j,k) \in \mathcal{E}} I^{m,n}_{i,j} \times I^{m,n}_{j,k} \times T_j (c^m_{i,j}, c^m_{j,k}) = \beta(m,n,i,j)\\
							T_n (\sum_{i:(i,n) \in \mathcal{E}} I^{m,n}_{i,n} \times c^m_{i,n}, r^{m,n}) )  =\gamma(m,n,i,j) \\ 
							\alpha(m,n,i,j) + \beta(m,n,i,j) + \gamma(m,n,i,j) \leq L^{m,n} \forall m,n \in \mathcal{S}, m \neq n\\
							r^{m,n} \leq R^{m,n}, \forall m,n \in \mathcal{S}, m \neq n \\
							I^{m,n}_{i,j} = \{0,1\} \forall m,n \in \mathcal{S}, m \neq n, (i,j) \in \mathcal{E}\\
						\end{array}
			\end{array}
			\nonumber
			\label{eqn:optimization}
	\end{equation}
	
	where 
	\begin{equation}
		b^{m,n}_j = \left\{
					\begin{array}{l}
						-1, \qquad if \quad j = m \\
						1, \qquad if \quad j = n \\
						0, \qquad otherwise  \\
					\end{array}
					\nonumber
					\right.
	\end{equation}

Constraints (1) describes the flow conservation conditions. Constraints (2) guarantees the actual bit rates originating from sender $m$ contains all the lower rated sessions destined for each receivers on each link. Constraints (3) requires the aggregate link rates should not exceed the link capacity. Constraints (4) means the aggregate latency for each session should not violate the maximal bearable one. The first parts are the link latencies, the second parts are the by-passing transcoding latencies at intermediate surrogates while the last part is the last-mile transcoding latency caused at the receivers' surrogate.

